Comparison and Bayesian Estimation of Feature Allocations

Feature allocation models postulate a sampling distribution whose parameters are derived from shared features. Bayesian models place a prior distribution on the feature allocation, and Markov chain Monte Carlo is typically used for model fitting, which results in thousands of feature allocations sampled from the posterior distribution. Based on these samples, we propose a method to provide a point estimate of a latent feature allocation. First, we introduce FARO loss, a function between feature allocations which satisfies quasi-metric properties and allows for comparing feature allocations with differing numbers of features. The loss involves finding the optimal feature ordering among all possible, but computational feasibility is achieved by framing this task as a linear assignment problem. We also introduce the FANGS algorithm to obtain a Bayes estimate by minimizing the Monte Carlo estimate of the posterior expected FARO loss using the available samples. FANGS can produce an estimate other than those visited in the Markov chain. We provide an investigation of existing methods and our proposed methods. Our loss function and search algorithm are implemented in the fangs package in R.

==> psm.tex <==
There is also a potential basis for loss functions related to feature allocations that relies on adjacency matrices and the pairwise similarity matrix. For simplicity, notation is selected in consistency with the same concepts used to describe partition loss in \citet{caviarpd}. We denote the adjacency matrix as $\gamma (Z)$ and the pairwise similarity matrix (or PSM) as $\Psi$.

The adjacency matrix is a way of converting the feature allocation into a notation that keeps track of the number of shared features for each pair of items being allocated. The adjacency matrix (given $ Z $) is defined as the product $ \gamma(Z) = ZZ' $ (simply $ Z $ multiplied by its transpose). This matrix will have dimensions $n\times n$, where $ n $ is the number of items being allocated. If the $i,j$ element of this adjacency matrix is $u$, that means that items $i$ and $j$ share $u$ features. The pairwise similarity matrix is then constructed by taking the element-wise average of multiple adjacency matrices, displaying a matrix containing the ``average number of shared features'' across all samples. For example, if we have $B$ samples from a feature allocation distribution, we simply add up all $ B $ adjacency matrices and divide by $ B $ to get the pairwise similarity matrix, as seen in Equation \ref{eq:psm}.

\begin{equation}
    \Psi_{i,j} = \frac{1}{B}\sum_{t=1}^B \gamma_{i,j} (Z^{(t)})
    \label{eq:psm}
\end{equation}

Consider the following example to see how feature allocation matrices (in $Z$ notation) relate to the corresponding adjacency matrices and pairwise similarity matrix. Figure \ref{fig:z_matrices} shows three unique feature allocations $ \{Z_1, Z_2, Z_3 \} $, as well as their corresponding adjacency matrices. These adjacency matrices show the number of shared features between items in the feature allocations. Figure \ref{fig:psm} shows the pairwise similarity matrix associated with the same three feature allocations. This pairwise similarity matrix gives an idea as to which items share many features on average and which share few features on average.

\begin{figure}[tb]
    \begin{center}
        $ Z_1 =
        \setlength\arraycolsep{2.5pt}
        \begin{bmatrix}[name=A]
            0 & 0 & 0 & 1 \\
            \rowcolor{yellow!40}
            0 & \mathbf{1} & \mathbf{1} & 0 \\
            1 & 1 & 1 & 0 \\
            1 & 1 & 1 & 1 \\
            0 & 0 & 1 & 0 \\
            1 & 0 & 1 & 0
        \end{bmatrix} 
        \hspace{0.3cm} \Longrightarrow \hspace{0.3cm}
        Z_1 Z_1^\prime = 
        \begin{bmatrix}[name=B]
            1 & 0 & 0 & 1 & 0 & 0 \\
            0 & \colorbox{yellow!40}{$2$} & 2 & 2 & 1 & 1 \\
            0 & 2 & 3 & 3 & 1 & 2 \\
            1 & 2 & 3 & 4 & 1 & 2 \\
            0 & 1 & 1 & 1 & 1 & 1 \\
            0 & 1 & 2 & 2 & 1 & 2
        \end{bmatrix}$
        \tikz [remember picture, overlay] \draw [blue,->] (A-2-4) to [bend left=45] (B-2-2) ;

        \vspace{0.5cm} 

        $ \, \, Z_2 = 
        \setlength\arraycolsep{2.5pt}
        \begin{bmatrix}[name=C]
            1 & 1 & 0 & 0 \\
            \rowcolor{yellow!40}
            1 & 0 & 1 & \mathbf{1} \\
            0 & 1 & 1 & 1 \\
            1 & 1 & 0 & 1 \\
            \rowcolor{yellow!40}
            0 & 1 & 0 & \mathbf{1} \\
            1 & 1 & 0 & 1 
        \end{bmatrix} \hspace{0.3cm} \Longrightarrow \hspace{0.3cm}
        Z_2 Z_2^\prime = 
        \begin{bmatrix}[name=D]
            2 & 1 & 1 & 2 & 1 & 2 \\
            1 & 3 & 2 & 2 & 1 & 2 \\
            1 & 2 & 3 & 2 & 2 & 2 \\
            2 & 2 & 2 & 3 & 2 & 3 \\
            1 & \colorbox{yellow!40}{$1$} & 2 & 2 & 2 & 2 \\
            2 & 2 & 2 & 3 & 2 & 3
        \end{bmatrix}$
        \tikz [remember picture, overlay] \draw [blue,->] (C-2-4) to [bend left=65] (D-5-2) ;
        \tikz [remember picture, overlay] \draw [blue,->] (C-5-4) to [bend left=65] (D-5-2) ;
        
        \vspace{0.5cm} 

        $ Z_3 = \,
        \setlength\arraycolsep{2.5pt}
        \begin{bmatrix}[name=E]
            0 & 1 & 1 \\
            1 & 1 & 1 \\
            0 & 0 & 0 \\
            0 & 1 & 0 \\
            0 & 1 & 0 \\
            0 & 1 & 0 
        \end{bmatrix} \hspace{0.24cm} \Longrightarrow \hspace{0.3cm}
        Z_3 Z_3^\prime = \,
        \begin{bmatrix}[name=F]
            2 & 2 & 0 & 1 & 1 & 1 \\
            2 & 3 & 0 & 1 & 1 & 1 \\
            0 & 0 & 0 & 0 & 0 & 0 \\
            1 & 1 & 0 & 1 & 1 & 1 \\
            1 & 1 & 0 & 1 & 1 & 1 \\
            1 & 1 & 0 & 1 & 1 & 1
        \end{bmatrix}$
        
    \end{center}
    \caption{Three examples of feature allocations (left) and their corresponding adjacency matrices (right), which are symmetric. Note that the diagonal element $(i,i)$ of the adjacency matrix shows how many features are allocated to the $i$th observation (see observation 2 of $Z_1$). The off-diagonal element $(i,j)$ represents how many elements observations $i$ and $j$ share (see observations 2 and 5 of $Z_2$).}
    \label{fig:z_matrices}
\end{figure}


\begin{figure}[tb]
    \centering
    \[\left[\begin{array}{cccccc}
     1.67 & 1.00 & 0.33 & 1.33 & 0.67 & 1.00 \\
     1.00 & 2.67 & 1.33 & 1.67 & 1.00 & 1.33 \\
     0.33 & 1.33 & 2.00 & 1.67 & 1.00 & 1.33 \\
     1.33 & 1.67 & 1.67 & 2.67 & 1.33 & 2.00 \\
     0.67 & 1.00 & 1.00 & 1.33 & 1.33 & 1.33 \\
     1.00 & 1.33 & 1.33 & 2.00 & 1.33 & 2.00
    \end{array}\right]\]
    \caption{The pairwise similarity matrix corresponding to the feature allocations and adjacency matrices shown in Figure \ref{fig:z_matrices}. It is simply the element-wise average of the three adjacency matrices.}
    \label{fig:psm}
\end{figure}

We introduce the concept of the pairwise similarity matrix here because \citet{lui2021} used it to construct a least-squares loss function used in feature allocation estimation for cytometry data. For a terminology comparison, we refer to their ``mean adjacency matrix'' as the pairwise similarity matrix $\Psi$. In this cytometry study, the loss function used to estimate $\hat{Z}$ was:

$$ \hat{Z} = \underset{Z}{\text{argmin}} \sum_{i=1}^n \sum_{j=1}^n (\gamma_{i,j}(Z) - \Psi_{i,j})^2 $$

However, while both the adjacency matrix (for a particular feature allocation) and the pairwise similarity matrix (for a set of samples from a feature allocation distribution) have a useful intuition related to the number of shared features, there is at least one major drawback in using this notation both for representing feature allocations and as a loss function to summarize a set of samples. This comes from the fact that the adjacency matrix is not guaranteed to be a unique representation of a distinct feature allocation $Z$. More technically, the space of all unique feature allocations does not have a one-to-one mapping with the space of all adjacency matrices implied by those same feature allocations. Each feature allocation maps to one and only one adjacency matrix, but each adjacency matrix does not necessarily map to one and only one feature allocation.

This leads to a major issue when using a loss based on the adjacency matrices or pairwise similarity matrix. A particular adjacency matrix could be found as the optimal estimate given a particular criterion, but this adjacency matrix could map back to multiple distinct feature allocations. It would then be a random guess as to which of these feature allocations is actually more representative of the samples, as any loss based on the adjacency matrices would treat them identically.


\textcolor{red}{From Dr. Warr: } \\
Regarding the shared column space, if we fix features $F_1, F_2, F_3$ associated with $Z_1$ and have the model $u_i = F_1*Z_1[i,1] + F_2*Z_1[i,2] +F_3*Z_1[i,3]$, then there exist features $G_1, G_2, G_3, G_4$ associated with  $Z_2$ where $v_i = G_1*Z_2[i,1] + G_2*Z_2[i,2] +G_3*Z_2[i,3]+G_4*Z_2[i,4] $ such that $u_i = v_i$ for all $i \in \{1, \ldots , 6\}$.

\textcolor{blue}{Added by Jacob in regards to the column space question (may or may not be necessary - what do you guys think?):} \\
If we look more closely at $Z_1$ and $Z_2$ in the example in Figure \ref{fig:ZmatVsAdjMat}, perhaps they are more similar than originally thought. For instance, item $i$ has the exact same number of features in $Z_1$ and $Z_2$ for $i = 1,2,\ldots,6$. Also, items $i$ and $j$ share the exact same number of features in $Z_1$ and $Z_2$ for $i,j = 1,2,\ldots,6$. These properties should follow intuitively by the definition of the adjacency matrix. Why is it then that $Z_1$ and $Z_2$ appear to be so different at first glance? The answer lies in the choice of equivalence class. The columns of $Z_1$ can be expressed as a linear combination of the columns of $Z_2$ (and vice versa). If the equivalence class was loosened to equate any two matrices with the same column space, then $Z_1$ and $Z_2$ would actually be considered equivalent, and thus there would be no issue with them mapping to the same adjacency matrix. It can also be shown that two feature allocation matrices with the same column space map to the same adjacency matrix using properties of isomorphism \citep{isomorphism}. The idea of defining an equivalence class based on shared column space could certainly be worth investigating in the context of a linear latent feature model, but that is not the aim of our current analysis. Moreover, none of these properties would necessarily hold in a more general latent feature model where nonlinear features may be present \citep{gundersen-nonlinear}.

Regardless of this discussion, we are applying the left-ordering equivalence class in this paper \citep{griffithsIBP}. Therefore, although the matrices $Z_1$ and $Z_2$ in our example are equivalent in terms of their column space, they are still not considered equivalent by their left-ordering. As pointed out previously, $Z_1$ and $Z_2$ have different numbers of features, and no two columns are identical between them, so key differences are still present. In summary, the lack of a one-to-one mapping with the adjacency matrix is still an issue under the left-ordering equivalence class, and a loss function defined on the feature allocation matrix itself is desirable.

